NuSTAR Tests of Sterile-Neutrino Dark Matter: New Galactic Bulge Observations and Combined Impact

We analyze two dedicated NuSTAR observations with exposure ${\sim}190$ ks located ${\sim}10^\circ$ from the Galactic plane, one above and the other below, to search for x-ray lines from the radiative decay of sterile-neutrino dark matter. These fields were chosen to minimize astrophysical x-ray backgrounds while remaining near the densest region of the dark matter halo. We find no evidence of anomalous x-ray lines in the energy range 5--20 keV, corresponding to sterile neutrino masses 10--40 keV. Interpreted in the context of sterile neutrinos produced via neutrino mixing, these observations provide the leading constraints in the mass range 10--12 keV, improving upon previous constraints in this range by a factor ${\sim}2$. We also compare our results to Monte Carlo simulations, showing that the fluctuations in our derived limit are not dominated by systematic effects. An updated model of the instrumental background, which is currently under development, will improve NuSTAR's sensitivity to anomalous x-ray lines, particularly for energies 3--5 keV.

==> model_table.tex <==
\begin{table*}[t]
\centering
\caption{The \nustar{} spectral model used in this paper. Parameters with numerical values are frozen to those values, and all free parameters are allowed to vary independently between FPMA/B and between the two obsIDs.}
\begin{tabularx}{\textwidth}{CCCD}
\hline
\hline
& & & \\
 Model component & \textsc{xspec} model\footnote{The CXB, GRXE, and DM line models also include absorption from the interstellar medium through the \texttt{tbabs} model with fixed column density $N_\text{H}$, as well as absorption from the beryllium x-ray shield. All model components except the internal continuum include the absorption effects of detector surface material. See Sec.~\ref{sec:spect_fit} for details.} &  Parameter  & Value \\
& & & \\
\hline \\
%  & $\ell,\,b$ (deg) & FPMA / B (ks) & FPMA / B (cm$^2$) & FPMA / B (deg$^2$) \\
%  \hline
%   40410001002 & 355.2354,\: $+$10.8656  & 54.6 / 54.2 & {12.40 / 12.28} & {4.48 / 4.53} \\
% 40410002002 &  6.8695, \,\,\,-9.9771 & 48.7 / 48.5 & {12.71 / 12.60}  & {4.53 / 4.56}  \\
 CXB & \texttt{powerlaw}*\texttt{highecut} & 3--20 keV flux & $2.6\times 10^{-11}\text{\,erg\,s}^{-1}\text{\,cm}^{-2}\text{\,deg}^{-2}$ \cite{Gruber:1999,Churazov:2006bk}
 \\
  & & Spectral index $\Gamma$ & $1.29$ \cite{Gruber:1999,Churazov:2006bk} \\
  & & $E_\text{cut}$ & $10^{-4}\text{\,keV}$ \\
  & & $E_\text{fold}$ & $40$ keV \cite{Gruber:1999,Churazov:2006bk} \\
  & & &  \\
 GRXE & \texttt{apec} & 3--20 keV flux & Free \\
 & & Plasma $kT$ & 8 keV \cite{Kaneda:1997,Yuasa:2012,Perez:2019a} \\
 & & Abundance ratio & Free within 0--1.2 \\
 & & & \\
 Internal continuum & \texttt{bknpower} & $E_\text{break}$ & 124 keV \cite{Wik:2014} \\
 & & $\Gamma(E < E_\text{break})$ & $-0.05$ \cite{Wik:2014}\\
 & & $\Gamma(E > E_\text{break})$ & $-0.85$ \cite{Wik:2014} \\
 & & Normalization & Free \\
 & & & \\
 Internal power-law & \texttt{powerlaw} & Spectral index $\Gamma$ & Frozen for each FPM/obsID (Sec.~\ref{sec:spect_fit}) \\
 & & Relative norm. & Frozen for each FPM/obsID (Sec.~\ref{sec:spect_fit})\\
 & & & \\
 Internal lines & \texttt{lorentz} & Line energies & 10.2, 19.7, 104.5 keV \cite{Wik:2014}\\
 & & Line widths & 0.6, 0.2, 0.5 keV \cite{Wik:2014}\\
 & & Line norms. & Free \\
 & & & \\
 DM line & \texttt{gaussian} & Line energy & See Sec.~\ref{sec:spect_fit} \\
  & & Line width & 0 keV \\
 & & Line flux & See Sec.~\ref{sec:spect_fit} \\
 \hline
 \hline
\end{tabularx}
 \label{model_table}
\end{table*}
